Non-classical effects in wave packet dynamics

Treating the ideal coherent state as a reference state, the effects due to departure from coherence of an initial wave packet propagating through a nonlinear medium, were examined, specifically in the context of non-classical effects such as revivals, fractional revivals, squeezing and higher-order squeezing during its temporal evolution. Further, these studies were extended to examine the role of quantum entanglement in bipartite systems. The dynamics of quantum expectation values were tracked carefully in various cases and the conditions under which a wave packet spreads chaotically, were investigated.

==> adaggerrarpluss.tex <==
\chapter{Expression for $\aver{a^{\dagger r} a^{r+s}}$ at time $t$
for an initial PACS $\ket{\alpha,m}$ governed by the Hamiltonian
$H=\hbar\chi N(N-1) \,\,(N=a^{\dagger} a)$ }
\label{generalform}
The initial state $\ket{\psi(0)}$ is the PACS $\ket{\alpha,m}$.
Then the state at a later time $t$ is given by 
\begin{equation}
\ket{\psi(t)}=e^{-i\chi N(N-1)}\ket{\alpha,m}
\end{equation}
Hence,
\begin{eqnarray}
&\expect{\psi(t)}{a^{\dagger r} a^{r+s}}{\psi(t)}&
=\sum_{l=0}^{\infty}\sum_{n=0}^{\infty}\sum_{u=0}^{\infty}
\sum_{v=0}^{\infty}\inner{\alpha,m}{l}\,
\bra{l}e^{i\chi N(N-1)t}\ket{n}\nonumber\\
&&\times\bra{n}a^{\dagger r} a^{r+s}\ket{u}\,\bra{u}e^{-i\chi N(N-1)t}
\ket{v}\,\inner{v}{\alpha,m}
\end{eqnarray}
where complete sets of states
\begin{equation}
\sum_{l=0}^{\infty}\ket{l}\bra{l}=1\nonumber
\end{equation}
have been intriduced at appropriate places. On using 
\begin{equation}
a^p\ket{u}=\big(\frac{u!}{(u-p)!}\big)^{1/2}\ket{u-p}\nonumber
\end{equation}
and the orthogonal property of basis states the expression simplifies to 
\begin{eqnarray}
&=&
\sum_{l=0}^{\infty}
\Big[\frac{(l+s)!}{l!}\Big]^{1/2}\frac{l!}{(l-r)!}
\,e^{-i\chi \big((l+s)(l+s-1)-l(l-1)\big)t}
\inner{\alpha,m}{l}\inner{l+s}{\alpha,m}\nonumber\\
\end{eqnarray}
Expanding $\ket{\alpha,m}$ in the Fock basis we can see that 
\begin{equation}
\inner{\alpha,m}{l}=\big(\frac{m!^{\,2}}{(m-l)!}\big)^{1/2}\alpha^{*(m-1)}
e^{-\nu/2}
\end{equation}
Hence, we now have 
\begin{eqnarray}
\expect{\psi(t)}{a^{\dagger r} a^{r+s}}{\psi(t)}&=&\frac{e^{-\nu}}{m!L_m(-\nu)}\sum_{l=0}^{\infty}
\frac{l!}{(l-r)!}\frac{(l+s)!}{(l+s-m)!}
\frac{\alpha^s\,\nu^{l-m}}{(l-m)!}\nonumber\\
&\times&e^{-i\chi s(s-1)\,t}\,e^{-2i\chi ls\,t}
\end{eqnarray}
But, 
\begin{equation}
\frac{(l+s)!}{(l+s-m)!}\,\,\nu^{l-m}=\nu^{-s}\frac{d^m}{d\nu^m}(\nu^{l+s})
\end{equation}
Using this it follows that
\begin{eqnarray}
\expect{\psi(t)}{a^{\dagger r} a^{r+s}}{\psi(t)}&=&\frac{\alpha^s e^{-\nu}e^{-i\chi\,s(s-1)t}}{\nu^ s L_m(-\nu)m!}
\sum_{l=0}^{\infty}\frac{l!}{(l-r)!}\frac{e^{-2i\chi \,lst}}{(l-m)!}
\frac{d^m}{d\nu^m}(\nu^{l+s})\nonumber\\
&=&\frac{\alpha^s e^{-\nu}e^{-i\chi\,s(s-1)t}}{\nu^ s L_m(-\nu)m!}
\sum_{l=0}^{\infty}\frac{e^{-2i\chi \,lst}}{(l-m)!}\frac{d^m}{d\nu^m}
\Big(\nu^{r+s}\frac{d^{\,r}\nu^l}{d\nu^r}\Big)
\end{eqnarray}
which can be simplified to 
\begin{eqnarray}
&=&
\frac{\alpha^s e^{-\nu}}{\nu^sL_m(-\nu)m!}
\sum_{l=0}^{m}\binom{m}{l}\Big(\frac{d^l\nu^{r+s}}{d\nu^l}\Big)
\sum_{n=r-l}^{r-l+m}\binom{r-l+m}{n}\frac{m!}{(n-r+l)!}\nonumber\\
&\times&\nu^{n-r+l}e^{-2i\chi nst}e^{-i\chi(s(s-1)+2ms )t}
\exp(\nu e^{-2i\chi st}).
\end{eqnarray}


Note: for $m=0$, we retrive Eq. (\ref{nthmoment}) corresponds to an initial 
CS $\ket{\alpha}$.

